Conversion-Based Dynamic-Creative-Optimization in Native Advertising

Yahoo Gemini native advertising marketplace serves billions of impressions daily, to hundreds millions of unique users, and reaches a yearly revenue of many hundreds of millions USDs. Powering Gemini native models for predicting advertise (ad) event probabilities, such as conversions and clicks, is OFFSET - a feature enhanced collaborative-filtering (CF) based event prediction algorithm. The predicted probabilities are then used in Gemini native auctions to determine which ads to present for every serving event (impression). Dynamic creative optimization (DCO) is a recent Gemini native product that was launched two years ago and is increasingly gaining more attention from advertisers. The DCO product enables advertisers to issue several assets per each native ad attribute, creating multiple combinations for each DCO ad. Since different combinations may appeal to different crowds, it may be beneficial to present certain combinations more frequently than others to maximize revenue while keeping advertisers and users satisfied. The initial DCO offer was to optimize click-through rates (CTR), however as the marketplace shifts more towards conversion based campaigns, advertisers also ask for a {conversion based solution. To accommodate this request, we present a post-auction solution, where DCO ads combinations are favored according to their predicted conversion rate (CVR). The predictions are provided by an auxiliary OFFSET based combination CVR prediction model, and used to generate the combination distributions for DCO ad rendering during serving time. An online evaluation of this explore-exploit solution, via online bucket A/B testing, serving Gemini native DCO traffic, showed a 53.5% CVR lift, when compared to a control bucket serving all combinations uniformly at random.

==> plot1.tex <==
\begin{figure}[!htb]
\centering
\begin{tikzpicture}
  \begin{axis}[
  	xlabel = {$Time$ $[days]$},
    ylabel = {$Lift$ $[\%]$},
    xmin=0, xmax=115,
    ymin=0, ymax=0.8,
    ymajorgrids=true,
    xmajorgrids=true,
    height=5cm, width=8.5cm,
    legend style={at={(0.75,0.97)}}
]
\addplot [
    color=red,
    mark=*,
] coordinates {
      (0,-0.01)
(1,0.06)
(2,0.17)
(3,0.25)
(4,0.37)
(5,0.46)
(6,0.52)
(7,0.58)
(8,0.6)
(9,0.62)
(10,0.61)
(11,0.63)
(12,0.63)
(13,0.63)
(14,0.62)
(15,0.59)
(16,0.57)
(17,0.57)
(18,0.55)
(19,0.54)
(20,0.53)
(21,0.52)
(22,0.5)
(23,0.46)
(24,0.47)
(25,0.45)
(26,0.41)
(27,0.43)
(28,0.42)
(29,0.4)
(30,0.39)
(31,0.42)
(32,0.4)
(33,0.4)
(34,0.4)
(35,0.38)
(36,0.36)
(37,0.36)
(38,0.35)
(39,0.09)
(40,0.16)
(41,0.22)
(42,0.31)
(43,0.25)
(44,0.37)
(45,0.24)
(46,0.05)
(47,0.13)
(48,0.23)
(49,0.22)
(50,0.16)
(51,0.23)
(52,0.28)
(53,0.24)
(54,0.14)
(55,0.17)
(56,0.2)
(57,0.11)
(58,0.2)
(59,0.16)
(60,0.14)
(61,0.19)
(62,0.18)
(63,0.08)
(64,0.23)
(65,0.21)
(66,0.33)
(67,0.33)
(68,0.37)
(69,0.38)
(70,0.38)
(71,0.4)
(72,0.42)
(73,0.42)
(74,0.43)
(75,0.44)
(76,0.44)
(77,0.43)
(78,0.44)
(79,0.44)
(80,0.45)
(81,0.46)
(82,0.48)
(83,0.47)
(84,0.48)
(85,0.48)
(86,0.5)
(87,0.51)
(88,0.48)
(89,0.46)
(90,0.46)
(91,0.46)
(92,0.39)
(93,0.49)
(94,0.46)
(95,0.44)
(96,0.45)
(97,0.42)
(98,0.4)
(99,0.4)
(100,0.4)
(101,0.39)
(102,0.4)
(103,0.38)
(104,0.36)
(105,0.32)
(106,0.34)
(107,0.33)
(108,0.35)
(109,0.38)
(110,0.33)
(111,0.41)
(112,0.4)
(113,0.43)
(114,0.44)
(115,0.41)
    };
\addlegendentry{LogLoss}
\addplot [
    color=blue,
    mark=*
] coordinates {
(0,-0.02)
(1,0.02)
(2,0.12)
(3,0.19)
(4,0.29)
(5,0.39)
(6,0.46)
(7,0.48)
(8,0.53)
(9,0.6)
(10,0.58)
(11,0.56)
(12,0.54)
(13,0.55)
(14,0.53)
(15,0.53)
(16,0.53)
(17,0.51)
(18,0.52)
(19,0.48)
(20,0.46)
(21,0.47)
(22,0.49)
(23,0.44)
(24,0.43)
(25,0.41)
(26,0.41)
(27,0.37)
(28,0.39)
(29,0.37)
(30,0.37)
(31,0.37)
(32,0.35)
(33,0.35)
(34,0.36)
(35,0.34)
(36,0.35)
(37,0.36)
(38,0.33)
(39,0.29)
(40,0.32)
(41,0.37)
(42,0.51)
(43,0.41)
(44,0.5)
(45,0.24)
(46,0.11)
(47,0.16)
(48,0.23)
(49,0.24)
(50,0.17)
(51,0.25)
(52,0.26)
(53,0.22)
(54,0.13)
(55,0.18)
(56,0.21)
(57,0.13)
(58,0.18)
(59,0.16)
(60,0.14)
(61,0.18)
(62,0.18)
(63,0.13)
(64,0.16)
(65,0.16)
(66,0.24)
(67,0.24)
(68,0.29)
(69,0.28)
(70,0.29)
(71,0.3)
(72,0.31)
(73,0.31)
(74,0.33)
(75,0.35)
(76,0.34)
(77,0.36)
(78,0.35)
(79,0.35)
(80,0.34)
(81,0.37)
(82,0.39)
(83,0.37)
(84,0.38)
(85,0.37)
(86,0.41)
(87,0.41)
(88,0.39)
(89,0.35)
(90,0.39)
(91,0.39)
(92,0.32)
(93,0.41)
(94,0.36)
(95,0.36)
(96,0.39)
(97,0.37)
(98,0.36)
(99,0.37)
(100,0.37)
(101,0.37)
(102,0.37)
(103,0.37)
(104,0.37)
(105,0.33)
(106,0.32)
(107,0.31)
(108,0.35)
(109,0.35)
(110,0.33)
(111,0.37)
(112,0.37)
(113,0.37)
(114,0.36)
(115,0.37)
    };
\addlegendentry{sAUC}
  \end{axis}
\end{tikzpicture}
\caption{Offline LogLoss and stratified AUC (sAUC) lifts of DLFM model over the baseline model vs. time.}
\label{fig: offline lifts}
\end{figure}

==> plot2.tex <==
\begin{figure}[!htb]
\centering
\begin{tikzpicture}
  \begin{axis}[
  	xlabel = {$Time$ $[days]$},
    ylabel = {$Lift$ $[\%]$},
    legend pos=north west,
    xmin=0, xmax=7,
    ymin=0, ymax=4,
    ymajorgrids=true,
    xmajorgrids=true,
    height=5cm, width=8.5cm,
    legend style={at={(0.5,0.97)}}
]
\addplot [
    color=red,
    mark=*,
] coordinates {
(0,2.47645484726637)
(1,0.586511023373393)
(2,2.17624426449665)
(3,1.53153466784846)
(4,0.576215325006801)
(5,0.798074021310935)
(6,2.05588388628037)
(7,1.45082031750359)
    };
\addlegendentry{CPM}
\addplot [
    color=blue,
    mark=*
] coordinates {
(0,1.45889627997642)
(1,2.49896122542719)
(2,3.4159403748109)
(3,2.45624022601003)
(4,1.69509960524661)
(5,2.22810565717115)
(6,1.72489162925449)
(7,1.70178844640789)
    };
\addlegendentry{CTR}
  \end{axis}
\end{tikzpicture}
\caption{Online CPM and CTR lifts of DLFM bucket over the production bucket vs. time.}
\label{fig: online lifts}
\end{figure}

==> user_table.tex <==
\begin{table*}[ht!]
\scriptsize
\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|c||}{Feature} & \begin{sideways}\begin{tabular}[c]{@{}c@{}}article\\ topics \end{tabular} \end{sideways} &
\begin{sideways}\begin{tabular}[c]{@{}c@{}}app install\\ features \end{tabular} \end{sideways}& 
\begin{sideways}\begin{tabular}[c]{@{}c@{}}ctr per\\ advertiser \end{tabular} \end{sideways}& \begin{sideways}\begin{tabular}[c]{@{}c@{}}ctr per\\ category\end{tabular}  \end{sideways}& \begin{sideways}\begin{tabular}[c]{@{}c@{}}ctr per\\ campaign\end{tabular}  \end{sideways}& \begin{sideways}\begin{tabular}[c]{@{}c@{}}user\\ topics\end{tabular}  \end{sideways}& \begin{sideways}\begin{tabular}[c]{@{}c@{}}user\\ categories\end{tabular}  \end{sideways}& \begin{sideways}\begin{tabular}[c]{@{}c@{}}external\\ segments\end{tabular} \end{sideways}&
\begin{sideways}\begin{tabular}[c]{@{}c@{}}local\\ hour\end{tabular} \end{sideways} &
\begin{sideways}\begin{tabular}[c]{@{}c@{}}page\\ section\end{tabular}\end{sideways} &
\begin{sideways}\begin{tabular}[c]{@{}c@{}}publisher\\ id\end{tabular}\end{sideways} &
\begin{sideways}\begin{tabular}[c]{@{}c@{}}tech\\ segments\end{tabular} \end{sideways} &
\begin{sideways}state \end{sideways} &
\begin{sideways}\begin{tabular}[c]{@{}c@{}}user\\ involvement\end{tabular} \end{sideways} &
\begin{sideways}age \end{sideways}&
\begin{sideways}gender \end{sideways} & 
\begin{sideways}\begin{tabular}[c]{@{}c@{}}Yahoo! user\\ interests \end{tabular} \end{sideways}& 
\begin{sideways}\begin{tabular}[c]{@{}c@{}} additional user\\ interests \end{tabular} \end{sideways} \\ \hline \hline
article topics&\gradient{0.14}&\gradient{1.00}&\gradient{1.00}&\gradient{1.00}&\gradient{0.86}&\gradient{1.00}&\gradient{1.00}&\gradient{0.29}&\gradient{0.57}&\gradient{0.57}&\gradient{0.71}&\gradient{0.29}&\gradient{0.29}&\gradient{1.00}&\gradient{0.57}&\gradient{1.00}&\gradient{1.00}&\gradient{1.00}\\ \hline
app install features&&\gradient{0.14}&\gradient{1.00}&\gradient{0.86}&\gradient{1.00}&\gradient{1.00}&\gradient{0.57}&\gradient{0.14}&\gradient{0.00}&\gradient{1.43}&\gradient{0.71}&\gradient{1.00}&\gradient{0.43}&\gradient{0.57}&\gradient{0.57}&\gradient{0.57}&\gradient{0.43}&\gradient{1.00}\\ \hline
ctr per advertiser&&&\gradient{0.14}&\gradient{1.71}&\gradient{3.29}&\gradient{1.00}&\gradient{1.14}&\gradient{0.71}&\gradient{0.71}&\gradient{5.43}&\gradient{1.29}&\gradient{1.71}&\gradient{0.43}&\gradient{1.29}&\gradient{0.86}&\gradient{1.00}&\gradient{1.29}&\gradient{1.86}\\ \hline
ctr per category&&&&\gradient{0.14}&\gradient{0.86}&\gradient{0.86}&\gradient{1.00}&\gradient{0.71}&\gradient{0.00}&\gradient{1.00}&\gradient{0.14}&\gradient{1.14}&\gradient{0.00}&\gradient{0.86}&\gradient{0.43}&\gradient{0.43}&\gradient{0.71}&\gradient{1.00}\\ \hline
ctr per campaign&&&&&\gradient{0.14}&\gradient{0.86}&\gradient{1.14}&\gradient{0.14}&\gradient{0.00}&\gradient{4.14}&\gradient{1.00}&\gradient{1.14}&\gradient{0.00}&\gradient{0.57}&\gradient{0.43}&\gradient{0.43}&\gradient{0.00}&\gradient{0.71}\\ \hline
user topics&&&&&&\gradient{0.71}&\gradient{0.71}&\gradient{0.86}&\gradient{0.86}&\gradient{1.00}&\gradient{0.86}&\gradient{1.00}&\gradient{0.86}&\gradient{0.86}&\gradient{0.86}&\gradient{0.86}&\gradient{0.86}&\gradient{0.86}\\ \hline
user categories&&&&&&&\gradient{0.00}&\gradient{0.43}&\gradient{0.00}&\gradient{1.57}&\gradient{0.71}&\gradient{0.86}&\gradient{0.43}&\gradient{0.71}&\gradient{0.29}&\gradient{0.29}&\gradient{0.29}&\gradient{0.71}\\ \hline
external segments&&&&&&&&\gradient{0.14}&\gradient{0.14}&\gradient{1.14}&\gradient{0.14}&\gradient{1.14}&\gradient{0.00}&\gradient{0.14}&\gradient{0.14}&\gradient{0.14}&\gradient{0.86}&\gradient{0.71}\\ \hline
local hour&&&&&&&&&\gradient{0.00}&\gradient{1.00}&\gradient{0.00}&\gradient{0.43}&\gradient{0.29}&\gradient{0.29}&\gradient{0.14}&\gradient{0.00}&\gradient{0.29}&\gradient{0.00}\\ \hline
page section&&&&&&&&&&\gradient{0.14}&\gradient{0.57}&\gradient{6.00}&\gradient{3.00}&\gradient{1.57}&\gradient{1.57}&\gradient{1.57}&\gradient{1.43}&\gradient{1.57}\\ \hline
publisher id&&&&&&&&&&&\gradient{0.00}&\gradient{0.86}&\gradient{0.57}&\gradient{0.29}&\gradient{0.57}&\gradient{0.00}&\gradient{0.14}&\gradient{0.57}\\ \hline
tech segments&&&&&&&&&&&&\gradient{0.14}&\gradient{0.71}&\gradient{1.00}&\gradient{1.00}&\gradient{0.71}&\gradient{1.00}&\gradient{1.00}\\ \hline
state&&&&&&&&&&&&&\gradient{0.14}&\gradient{0.00}&\gradient{0.00}&\gradient{0.00}&\gradient{0.00}&\gradient{0.14}\\ \hline
user involvement&&&&&&&&&&&&&&\gradient{0.00}&\gradient{0.29}&\gradient{0.57}&\gradient{0.43}&\gradient{0.57}\\ \hline
age&&&&&&&&&&&&&&&\gradient{0.14}&\gradient{0.29}&\gradient{0.29}&\gradient{0.71}\\ \hline
gender&&&&&&&&&&&&&&&&\gradient{0.14}&\gradient{0.86}&\gradient{0.86}\\ \hline
Yahoo! user interests&&&&&&&&&&&&&&&&&\gradient{0.14}&\gradient{1.43}\\ \hline
additional user interests&&&&&&&&&&&&&&&&&&\gradient{0.14}\\ \hline
\end{tabular}
\caption{User vector normalized feature-allocation, several months after deploying DLFM into production, where darker colors indicate higher values.} 
\label{table: user structure}
\end{table*}
